Boundary Control for Suppressing Chaotic Response to Dynamic Hydrogen Blending in a Gas Pipeline

It is known that periodic forcing of nonlinear flows can result in a chaotic response under certain conditions. Such non-periodic and chaotic solutions have been observed in simulations of heterogeneous gas flow in a pipeline with periodic, time-varying boundary conditions. In this paper, we examine a proportional feedback law for boundary control of a parabolic partial differential equation system that represents the flow of two gases through a pipe. We demonstrate that periodic variation of the mass fraction of the lighter gas at the pipe inlet can result in the chaotic propagation of gas pressure waves, and show that appropriate flow control can suppress this response. We examine phase space solutions for the single pipe system subject to boundary control, and use numerical experiments to characterize conditions for the controller gain to suppress chaos.

==> ACNDC_2024_reviews.tex <==
Comments to author (Associate Editor)
=====================================

Three reviews were received. Please consider all the
comments of the reviewers.


Reviewer 1 of ACNDC 2024 submission 8

Comments to the author
======================

Summary: 

This paper presents an examination of a proportional
feedback law for boundary control of a parabolic PDE. The
authors provide scenarios that can result in chaotic
propagation of gas pressure waves and then using numerical
experiments provide conditions for the controller gain to
suprress chaos. 


Strengths: 

1. The paper is very well-written and logically. 

2. The problem is well motivated in the introduction
section and provides the reader sufficient background
before delving into the results. 

3. The methodology presented in the paper is systematic and
easy to follow. 

4. There is sufficient discussion on the results and the
examples help in reinforcing the main results. 

 
Suggestions:  

1. The authors mention that "a solution is chaotic if it is
highly sensitive to initial conditions". Is that the only
way a system can be chaotic? Several systems become chaotic
just with parameter variations. The authors should clarify
this. 

2. It would be nice to have some experimental validation to
the proposed results. 


Reviewer 2 of ACNDC 2024 submission 8

Comments to the author
======================

This paper deals with a new problem in the boundary control
 of chaotic dynamics in a distributed-parameter system
defined by partial differential equations.The contribution
is enough for a conference and the topic is relavant to the
conference. Thus, I recommend this paper to be accepted.

Reviewer 3 of ACNDC 2024 submission 8

Comments to the author
======================

This is essentially a simulation paper on a specific
application which is made interesting by the richness of
the dynamic behaviour. Overall the paper is well presented.

==> justification.tex <==
% \documentclass[10pt]{article}
% \usepackage{amsmath,amsfonts,amssymb,graphicx,color,psfrag}
% %\usepackage{concmath}
% \usepackage{url}
% \usepackage{palatino}
% %\usepackage{bibentry}
% \usepackage{enumerate}
% \usepackage{xcolor}
% \usepackage{soul}
% \usepackage{booktabs}
% \newcommand{\kprop}{\subscr{k}{prop}}

% \renewcommand{\baselinestretch}{1.05}
% \parskip = \medskipamount

%  \usepackage{relsize}
% \usepackage{vmargin}
% \setpapersize{USletter}
% \setmarginsrb{2.25cm}{2.25cm}{2.25cm}{2.25cm}
%                  {12pt}{20pt}{12pt}{36pt}

% \renewcommand{\theenumi}{(\roman{enumi})}
% \renewcommand{\labelenumi}{\theenumi}
% \renewcommand{\labelenumii}{\arabic{enumii})} 


% \newcommand{\referee}[1]{\;
%   \begin{minipage}[t]{.95\textwidth}
% %    ``{\small\color{blue} \textsc{#1}}''
% 	``{\color{blue}#1}''
%   \end{minipage}\medskip
%   }

% \newcommand{\refereebit}[1]{\; ``{\small\color{blue} \textsc{#1}}'' }
% \newcommand{\mc}{\mathcal}
% \newcommand{\mbb}{\mathbb}
% \newcommand{\real}{\mathbb R}
% \newcommand{\fvec}{\mathbf}
% \newcommand{\until}[1]{\{1,\dots,#1\}}
% \DeclareMathOperator*{\arcsinbf}{\mathrm{\bf arcsin}} 	  
% \newcommand{\vectorones}[1][]{\mathds{1}_{#1}}
% \newcommand{\vectorzeros}[1][]{\mathbbold{0}_{#1}}

% \newcommand{\todo}[1]{\par\noindent{\color{blue}\raggedright\textsc{#1}\par\marginpar{\large$\star$}}}
% \newcommand{\fdmargin}[1]{\marginpar{\color{red}\bf \tiny\ttfamily{FD:} #1}}
% \newcommand{\bpmargin}[1]{\marginpar{\color{violet}\bf \tiny\ttfamily{BP:} #1}}
% \newcommand{\sbmargin}[1]{\marginpar{\color{m}\bf \tiny\ttfamily{SB:} #1}}
% \newcommand{\note}[1]{ {\bf\color{red}$\fbox{Note:}$} #1\\}
% \newcommand{\tr}[0]{\color{red}}
% \newcommand{\tb}[0]{\color{blue}}
% \newcommand{\tg}[0]{\color{gray}}
% \newcommand{\tv}[0]{\color{violet}}
% \newcommand{\tm}[0]{\color{m}}

% \newcommand{\lr}[1]{\textcolor{red}{#1}}
% \newcommand{\edit}[1]{{\color{blue}{#1}}}

% \begin{document}


% %\nobibliography{../alias,../Main,../New,../FB}
% \bibliographystyle{unsrt}



% %%%%%%%%%%%%%%%%%%%%%%%%
% % title page
% %%%%%%%%%%%%%%%%%%%%%%%%

% \pagestyle{myheadings}
% %\thispagestyle{empty}

% % \markright{\small Report No. LA-UR-23-32580 \quad Boundary Control for Suppressing Chaotic Response to Dynamic Hydrogen Blending in a Gas Pipeline}

% %\headsep 0.5cm

% %\bigskip\bigskip


% \begin{center}
% {\bf \LARGE Abstract}
% \end{center}


% %\vspace*{2cm}

% %\today%%
% %\medskip

% \noindent \textbf{Report No. LA-UR-23-32580, Travel Request ID: 4CWW6} \\ 
% \noindent \textbf{Title:} \textit{Boundary Control for Suppressing Chaotic Response to Dynamic Hydrogen Blending in a Gas Pipeline}


% \noindent It is known that periodic forcing of nonlinear flows can result in a chaotic response under certain conditions.  Such non-periodic and chaotic solutions have been observed in simulations of heterogeneous gas flow in a pipeline with periodic, time-varying boundary conditions. In this talk, we examine a proportional feedback law for boundary control of a parabolic partial differential equation system that represents the flow of two gases through a pipe.  We demonstrate that periodic variation of the mass fraction of the lighter gas at the pipe inlet can result in the chaotic propagation of gas pressure waves, and show that  appropriate flow control can suppress this response.    We examine phase space solutions for the single pipe system subject to boundary control, and use numerical experiments to characterize conditions for the controller gain to suppress chaos. \\ \bigskip

% \noindent Luke Silas Baker \\
% \noindent $Z^{\#}$ 367475

% \thispagestyle{empty}


% \end{document}
